Fast and Versatile RNA Design via Motif-level Divide-and-Conquer and Structure-level Rival Search

RNA design aims to identify RNA sequences that fold into a target secondary structure. This task is challenging in terms of computational efficiency. Most existing methods focus on either minimum free energy (MFE)-based or ensemble-based metrics, leaving a gap for a unified approach that performs well across both. We introduce a fast and versatile RNA design algorithm inspired by our previous work on the undesignability of RNA structures and motifs (i.e., sets of contiguous structural loops). Our approach decomposes a target structure into a tree of sub-targets where each leaf node corresponds to a motif and each internal node corresponds to a substructure. We first design partial sequences for each motif, then these partial sequences are selectively and recursively combined via the cube pruning strategy borrowed from computational linguistics, enabling effective optimization of ensemble-based metrics. Finally, a novel whole-structure rival search further refines sequences to suppress misfolded alternatives and enhance MFE-based performance. Our method is highly efficient and also achieves state-of-the-art results on native RNAsolo structures and the Eterna100 benchmark, excelling in both ensemble- and MFE-based metrics. Additionally, it substantially improves the design of long-structure benchmark derived from 16S rRNA, increasing average folding probability from 0.18 to 0.39 with an order-of-magnitude speedup, demonstrating its effectiveness and scalability. Availability: Source code and data are available at: https://github.com/shanry/FastDesign.

==> Makefile <==
texbin=/Library/TeX/texbin
#texbin=/usr/local/texlive/2022/bin/universal-darwin
#texbin=/usr/local/texlive/2018/bin/x86_64-darwin
main:
	# rm -rf *.run.xml *.bcf *.aux *.out *.blg *.bbl *.log *.fls *.fdb_latexmk *~
	${texbin}/pdflatex main
	${texbin}/bibtex main
	if ${texbin}/bibtex siref; then \
		echo "seperate references\n"; \
	else \
		echo "combined references\n"; \
	fi
	${texbin}/pdflatex main
	${texbin}/pdflatex main
# supp:
# 	rm -rf *.run.xml *.bcf *.aux *.out *.blg *.bbl *.log *.fls *.fdb_latexmk *~
# 	${texbin}/pdflatex supp
# 	${texbin}/pdflatex supp       
split:
	yes | gs -dBATCH -sOutputFile="fastdesign.pdf" -dFirstPage=1 -dLastPage=9 -sDEVICE=pdfwrite main.pdf 
	yes | gs -dBATCH -sOutputFile="fastdesign.supp.pdf" -dFirstPage=10 -dAutoRotatePages=/None -sDEVICE=pdfwrite main.pdf  

clean:
	rm -rf  *.run.xml *.bcf *.bbl *.xwm *.aux *.out *.blg *.log *.fls *.fdb_latexmk main.pdf *~ 

fast:
	${texbin}/pdflatex main



==> ablation.tex <==
% !TEX root = main.tex
\subsection{Constrained Decoding}

\begin{figure}[h] 
    \centering
    \includegraphics[width=0.75\textwidth]{figs/combined_metrics_vs_length.pdf}
    \caption{Caption}
    \label{fig:combined_metrics_vs_length}
\end{figure}



==> conclusions.tex <==
% !TEX root = main.tex

\vspace{-0.2cm}
We have presented the first study of using autoregressive language models for RNA design (inverse folding).
Combining pretraining, constrained decoding, supervised learning, and reinforcement learning, our final model outperforms (or ties with) 
the state-of-the-art 
in ensemble-based metrics across all four datasets.
We also constructed and released comprehensive and carefully curated datasets for 
both training and testing, avoiding train-test contamination 
and ensuring high-quality training data, which will benefit future studies.


Our work can be improved in the following ways:
\vspace{-0.2cm}
\begin{itemize}
\item Our  decoding algorithm is sampling with context-free constraints. Since we need to sample a large amount of designs both for reinforcement learning and for testing, decoding speed 
%becomes the bottleneck in both. 
need improvement. First, we can use other decoding algorithms such as beam search \cite{huang+:2017}.
Secondly, the $\sim$30\% overhead due to constraints could be reduced by advanced techniques for LM generation of context-free languages \cite{dong+:2024}.
\item Currently,  reinforcement learning is 
still slow, limiting us to a small sample size. 
Once decoding speed improves, we can afford to 
do better reinforcement learning with more data and 
more exploration.
%\item We can explore a completely different model with a coupled variable approach, where each base-pair is decoded in one step, inspired by \cite{runge+:2019}. The advantage would be we no longer need constrained decoding.
\item Finally, we can explore Test-Time Reinforcement Learning (TTRL) methods
\cite{zuo+:2025} to train a different model for each testing structure, further exploiting test-time scaling.
\end{itemize}

==> dataset.tex <==
% !TEX root = main.tex

%\section{Dataset Filtering}
\vspace{-0.3cm}
\subsection{Test Dataset Construction (\Ytest)}

For RNA design, the test set \Ytest is a collection of target structures \vecystar.
We create a comprehensive test set consisting of four datasets, 
covering both manually-designed puzzles and native structures:

\begin{enumerate}
\item {\bf Eterna100} \cite{anderson+:2016}
is the standard and  most widely used benchmark for evaluating
RNA design programs. It contains 100 secondary structures
(i.e., human-designed ``puzzles'') of up to 400 \nts, varying in design difficulty from simple hairpins to intricate multiloop structures.


% \begin{figure}[t] 
%   \centering
%   \includegraphics[width=\linewidth]{figs/overview.png} % no extension needed usually
%   \caption{Caption for the figure.}
%   \label{fig:Overview}
% \end{figure}

\item {\bf Eterna100-v2} \cite{koodli2021redesigning}
modifies 19 puzzles from Eterna100 such that all puzzles are MFE-solvable
under the Turner 2004 energy model~\cite{mittal2024nndb} (using ViennaRNA v2~\cite{lorenz2011viennarna}).
%This dataset also contains solutions from Eterna players for all
%puzzles except for puzzle \#100 (whose solution is held out).

\item {\bf Rfam-Taneda-27} \cite{taneda:2011modena}
includes consensus secondary structures from seed alignments in Rfam 9.0,
with each entry corresponding to an RNA family. 

\item {\bf RNAsolo-100}, extracted from \cite{adamczyk2022rnasolo},
is a collection of secondary structures curated from a database of experimentally determined
RNA 3D structures. The specific ``100'' subset used here refers to 100 cleaned, non-redundant RNA structures we selected for secondary-structure-design benchmarking.
\end{enumerate}

\vspace{-0.2cm}
We call the set of unique structures from all four datasets our {\bf ``Union Test Set''}, notated \Ytest, which contains 246 unique structures, with length up to 400 \nts.

\vspace{-0.2cm}

\subsection{Supervised Learning Dataset Construction (\YXtrain)}
\label{sec:SLdata}

As mentioned above, our supervised training dataset \YXtrain is a set of $(\vecystar, \vecx)$ pairs where each \vecystar is a target structure (i.e., puzzle) and each \vecx is the corresponding RNA sequence (i.e., a design or solution).
We construct this set in four steps:
(a) collect the set of target structures (Sec.~\ref{sec:step1});
(b) filter out those that are too similar to the test structures to avoid test set contamination (Sec.~\ref{sec:step2});
(c) use SAMFEO to generate large amounts of candidate solutions for each remaining structure (Sec.~\ref{sec:step3});
and (d) filter those structures by quality (Boltzmann probability and ensemble defect) (Sec.~\ref{sec:step4}).
See Fig.~\ref{fig:workflow} for the workflow.


\subsubsection{Step 1: Collecting Raw Target Structures for Training (\Ytrainraw)}
\label{sec:step1}
\begin{figure*}%[t]
\centering
\vspace{-0.5cm}
\includegraphics[width=.99\linewidth]{figs/SL-filtering}
\caption{Workflow for constructing SL training data \YXtrain. 
\label{fig:workflow}}
\smallskip
\end{figure*}

We collect our training target structures from three sources:
\begin{itemize}
\item {\bf \Eternaweb}:
We downloaded the full collection of 22K player-designed structures (i.e., puzzles) from the Eterna website (\url{http://eternagame.org}), excluding those from Eterna100. We then removed structures longer than 500 \nts (to match  test sets) and undesignable ones,
which resulted in 18K  structures. 

\item {\bf \RfamlearnMFE}: This is the ``Rfam-Learn'' set from \cite{runge+:2019} with 65K structures. However, it is important to note that these are {\em \underline{not} native structures} from Rfam
but rather MFE structures (from ViennaRNA v2) of the {\em native sequences} from Rfam. Therefore, we renamed it to avoid confusion.
Note that these MFE structures are all designable by definition.

\item {\bf \RandomMFE}: To supplement the above human-designed and 
native-induced structures,
we want to include large amounts of artificial structures.
However, generating random secondary structures 
is problematic, as 
most of them will be undesignable.
Therefore, we first generated 100K random RNA sequences of lengths 100--500 \nts (with uniform distribution of $\{\nucA,\nucC,\nucG,\nucU\}$), and then use ViennaRNA v2 to compute their MFE structures. This way we made sure all of these structures are designable.
\end{itemize}


\vspace{-0.4cm}

\subsubsection{Step 2: Filtering out  \Ytrainraw structures that are too similar to test data (\Ytrain)}
\label{sec:step2}

% \begin{figure}[t] 
%   \centering
%   \includegraphics[width=\linewidth]{figs/final_filter_y.pdf} % no extension needed usually
%   \caption{Caption for the figure.}
%   \label{fig:filter_y}
% \end{figure}

To ensure the validity of any machine learning results, 
it is extremely important to avoid test set contamination,
otherwise we might get seemingly accurate results due to 
overfitting, i.e., the model simply memorizes the training data
and can not generalize to unseen data.
This has been a particularly serious issue in the machine learning for RNA literature, 
as pointed out by other researchers \cite{sato+:2021,szikszai+:2022}.
% 
%In supervised learning, if some structures \vecy in the training set \DSL
%$(\vecy, \vecx)$ is highly similar to that of the test set \vecyprime $\in$
%$\mathcal{Y}_{\text{test}}$, the model may memorize structure--sequence mappings 
%encountered during training. In such cases, evaluation on 
%$\mathcal{Y}_{\text{test}}$ would not accurately reflect the model’s 
%generalization ability but rather its capacity for memorization.

To ensure a rigorous evaluation, we removed training structures 
$\vecystar \in \Ytrainraw$ that were overly similar to any test structure 
$\vecy' \in \Ytest$. For each \vecystar, we computed a 
\textit{normalized minimum edit distance} that accounts for length differences:

\vspace{-20pt}
\[
d_{\text{min\_norm}}(\vecystar, \Ytest) =
\min_{\vecy' \in \Ytest}
\frac{d_{\text{edit}}(\vecystar, \vecy')}{\min(|\vecystar|, |\vecy'|)}.
\]
Here, $d_{\text{edit}}(\cdot, \cdot)$ denotes the edit distance between two structures, 
%$\vecy$ and $\vecy'$, 
and normalization by the length of the shorter structure 
$\min(|\vecystar|, |\vecy'|)$ ensures that our similarity measure 
is comparable across structures of different lengths. 
Training examples with $d_{\text{min\_norm}}(\vecystar, \Ytest)$ below a 
predefined threshold were excluded to eliminate 
similar structures 
and prevent information leakage between training and test sets.

But how to define the threshold? Here we propose a very simple method by measuring the distance between
 structures in \RandomMFE to those in the test set \Ytest,
 because presumably those artificial structures in the former should not be similar to anything in \Ytest.
As shown in Fig.~\ref{fig:threshold}(c),
the smallest normalized minimum edit distance between the two sets 
is over 0.2, so we choose 0.2 as a reasonable threshold
to filter other datasets (\Eternaweb and \RfamlearnMFE),
shown in Fig.~\ref{fig:threshold}(a--b).
After filtering, we have 16.2K structures remaining from \Eternaweb (2.1K filtered), 63.8K from \RfamlearnMFE (1.2K filtered), and 100K from \RandomMFE (none filtered).
These surviving structures form the \Ytrain set.



\vspace{-0.2cm}
% As we can see from the figure for 
\subsubsection{Step 3: Constructing Structure-Sequence Pairs (\YXtrainraw)}
\label{sec:step3}

To generate candidate designs for each target structure in \Ytrain, we use the state-of-the-art SAMFEO tool.
Specifically, for each structure in \Eternaweb, we generate
100 designs, for each structure in \RfamlearnMFE, we generate 20 designs, and for each structure in \RandomMFE, we generate 10 structures. Now we have a set \YXtrainraw of 1.6M+1.2M+1M=3.8M $(\vecystar, \vecx)$ pairs from the three data sources (see Fig.~\ref{fig:workflow}).

\begin{figure*}[t]%[t]
  \centering
  \hspace{-0.3cm}
  \begin{tabular}{ccc}
    \includegraphics[width=0.3\linewidth]{figs/eterna_y_filter.pdf}
    &
    \includegraphics[width=0.3\linewidth]{figs/rfam_y_filter.pdf}
    &
    \includegraphics[width=0.3\linewidth]{figs/random_y_filter.pdf}
    \\[-0.2cm]
    (a) $\Ytrainraw\_{\text{Eterna-web}}$
 & (b) $\Ytrainraw\_\text{Rfam-Learn-MFE}$ & (c) $\Ytrainraw\_{\text{Random-MFE}}$
  \end{tabular}
    \label{fig:SL+RL}
\caption{We remove \Ytrainraw structures which are similar to \Ytest to avoid contamination. 
We use  \RandomMFE  to derive the \dminnorm threshold of 0.2  (c) and apply it to \Eternaweb and \RfamlearnMFE (a--b).\label{fig:threshold}}\smallskip
\end{figure*}

%\paragraph{Generating Candidate Designs for Each Target Structure (from \Ytrain to \YXtrainraw)}

\subsubsection{Step 4: Filtering Structure-Sequence Pairs based on Quality (\YXtrain)}
\label{sec:step4}

To construct a reliable supervised learning (SL) dataset, we ensure that only high-quality 
%<<<<<<< HEAD
%structure--sequence pairs generated by SAMFEO are retained. For each target structure $\vecy$, 
%if SAMFEO produces $n$ candidate sequences $\vecx$, then the collection of all resulting 
%$(\vecy, \vecx)$ pairs for all $\vecy \in \Ytrain$ forms the set $\YXtrainraw$. However, not all 
% $(\vecy, \vecx) \in \YXtrainraw$ maybe of good quality. Therefore, we create a 
%filtered subset $\YXtrain \subseteq \YXtrainraw$ by retaining a structure--sequence pair 
%$(\vecy, \vecx)$ only if it satisfies the following criteria:
%=======
structure-sequence pairs generated by SAMFEO are retained. 
%For each target structure \vecy, 
%if SAMFEO produces $n$ candidate sequences \vecx, then the collection of all resulting 
%$(\vecy, \vecx)$ pairs for all $\vecy \in \Ytrain$ forms the set \YXtrainraw. However, not all 
% $(\vecy, \vecx) \in \YXtrainraw$ are of sufficient quality. Therefore, we construct a 
filtered subset for supervised learning,  $\YXtrain \subseteq \YXtrainraw$, by retaining a structure-sequence pair 
$(\vecystar, \vecx)$ only if it satisfies {\bf both} the following criteria:
%>>>>>>> overleaf-2025-11-21-0740

%To construct a reliable supervised learning (SL) dataset, we ensure that only high quality structure--sequence pairs generated by SAMFEO are retained. For each target structure \vecy, SAMFEO may produce multiple candidate sequences \vecx. However, not all sequences generated by SAMFEO are good-quality candidates for training a conditional language model. Therefore, we apply strict quality filters based on ensemble-level metrics. Specifically, we keep a structure--sequence pair (\vecy, \vecx) only if:

\begin{itemize}
    \item \textbf{Low normalized ensemble defect:}
    \(
        \mathrm{NED}(\vecx, \vecystar) \le 0.20,
    \)
    ensuring that, in equilibrium, at most 20\% of nucleotides deviate from the target structure.

    \item \textbf{Sufficient Boltzmann probability of the target structure:}
    \(
        p(\vecystar \mid \vecx) \ge 0.05,
    \)
    meaning that the target structure has at least a 5\% probability in the ensemble of all possible folds of \vecx.
\end{itemize}

Intuitively, $p(\vecystar \mid \vecx)$ measures how likely the designed sequence \vecx folds into the intended target structure \vecystar at thermodynamic equilibrium. Filtering with these thresholds removes sequences that do not reliably fold into the target structure or that strongly favor alternative competing folds.
After this filtering,
we have 1.3M pairs remaining from \Eternaweb,
among which we reserve 0.4M as a held set for hyperparameter tuning,
and the remaining 0.9M are used for training.
We also have 1.1M pairs and 1M pairs remaining from \RfamlearnMFE and \RandomMFE, respectively.
In total, the set \YXtrain has 3M $(\vecystar, \vecx)$ pairs (Fig.~\ref{fig:workflow}).






%
\vspace{-0.3cm}
\subsection{Selecting Structures for Reinforcement Learning (\YRL)}
\label{subsec:yrl_selection}

RL is computationally expensive because, for each target structure 
\(\vecystar \in \YRLraw\), where \(\YRLraw = \{\, \vecystar \mid (\vecystar, \vecx) \in \YXtrain \text{\, for some \vecx}\,\}\),
the model must generate many samples and evaluate their folding performance. 
Our goal is to identify a subset \(\YRL \subseteq \YRLraw\) for which RL is likely to yield meaningful improvement.


%\subsection{Selecting Structures for Reinforcement Learning ($\mathcal{Y}_{\mathrm{RL}}$)}
%\label{subsec:yrl_selection}


%To do so, we first decode the supervised-learning (SL) model trained on the full supervised dataset
%All \YXtrain. For each structure $\vec{y}$, we generate $K$ candidate sequences
%$\{x_k\}_{k=1}^K$ and compute their Boltzmann probabilities
%$p(y \mid x_k)$ using the RNA folding engine. We then summarize the distribution of these probabilities
%=======
To do so, we first decode structures in \YRLraw with the SL model trained on
 \YXtrain. For each structure $\vecystar \in \YRLraw$, we generate $K$ candidate sequences
$\{\vecx_k\}_{k=1}^K$ and compute their Boltzmann probabilities
$p(\vecystar \mid \vecx_k)$. We then summarize the distribution of these probabilities
with two statistics:

\begin{itemize}
  \item \textbf{Average probability (AoN):} \(\mathrm{AoN}(\vecystar) = \frac{1}{K}\sum_{k=1}^{K} p(\vecystar \mid \vecx_k)\), which reflects the performance of the SL model for structure in terms of the ensemble metric $p(\vecystar \mid \vecx_k)$.
\vspace{2mm}
  \item \textbf{Standard deviation of probabilities:}
  \(\mathrm{SD}(\vecystar) = \mathrm{Std}_k\!\left(p(\vecystar \mid \vecx_k)\right)\) capturing the variability, and hence the potential for improvement across sampled designs.
\end{itemize}

Using $\mathrm{SD}(\vecystar)$ alone can be misleading for structures whose probabilities remain uniformly low.
Thus, we use the \emph{normalized standard deviation} (NSD):
%\begin{equation}
 \( \mathrm{NSD}(\vecystar) = \frac{\mathrm{SD}(\vecystar)}{\mathrm{AoN}(\vecystar)},\)
%\end{equation}
which expresses variability relative to the mean probability and highlights structures where RL can exploit
useful diversity in folding outcomes.

\paragraph{Selection criteria.}
We select a structure $\vecystar \in \Ytrain$ for reinforcement learning if

\vspace{-8pt}
\begin{equation}
  \mathrm{AoN}(\vecystar) \ge 0.1
  \quad\text{and}\quad
  \mathrm{NSD}(\vecystar) > 0.5.
\end{equation}
The AoN threshold removes structures on which the SL model performs extremely poorly, while the NSD threshold ensures that there is sufficient variance among sampled sequences for RL to meaningfully refine the model. Applying both criteria yields a filtered subset \YRL of approximately 2.8K structures on which RL is both computationally feasible and empirically effective. Moreover, Figure 3 compares AoN scores before and after RL when training on either the full set \YRLraw or the filtered subset \YRL. When RL is applied to the entire \YRLraw, many structures $\vecystar \in \YRLraw$ actually exhibit degraded performance after RL. In contrast, when RL is restricted to \YRL, the model not only improves performance on most structures $\vecystar \in \YRL$ but also generalizes positively, yielding improvements for many structures in \YRLraw as well.



\begin{figure*}[t]
  \centering
  \hspace{-0.1cm}
  \begin{tabular}{ccc}
    \includegraphics[width=0.3\linewidth]{figs/summary_sd_vs_aon_probability.pdf}
    &
    \includegraphics[width=0.3\linewidth]{figs/summary_aon_pair1_probability.pdf}
    &
    \includegraphics[width=0.3\linewidth]{figs/summary_aon_pair2_probability.pdf}
    \\[-0.2cm]
    (a) Decoding \YRLraw using SL model & (b) RL on \YRL  & (c)   RL on \YRLraw
  \end{tabular}
  \vspace{-0.2cm}
  \label{tab:rl_data_selection}
\caption{Decoding results on \YRLraw using the SL model and the RL models trained on \YRL\ and \YRLraw.}
\end{figure*}


==> eval.tex <==
% !TEX root = main.tex
%\subsection{Pretraining}

\vspace{-0.4cm}
\subsection{Supervised Learning}
\vspace{-0.2cm}
%<<<<<<< HEAD

Figure~\ref{fig:sl_plot_with_table}(a) reports the best-of-$N$ Boltzmann probability achieved by each supervised-learning (SL) model as a function of the number of decoded samples $N$ per target structure. Across all sampling budgets, the pretrained Qwen-0.5B-SL model performs the strongest, reaching a best-of-$N$ probability of approximately $0.55$ at $N=10^4$. 
By contrast, both models trained from scratch, Qwen-0.5B-SL\_Scratch (decoder-only) and T5-0.7B-SL\_Scratch (encoder-decoder), perform substantially worse. %, with flatter curves and significantly lower probability values across all $N$. 
%This degradation is especially pronounced for the T5-scratch model, whose output remains near baseline even under extensive sampling. 
These results clearly suggest that training Transformer LMs for RNA design entirely from scratch is ineffective regardless of architecture. The \texttt{Target\_Initialization} 
is a simple baseline where for each unpaired position in \vecystar,
we use a distribution of 90\% \nucA\/ (other nucleotides 
for the remaining 10\%)
and for each basepair in \vecystar,
we use a distribution of 70\% \nucG\nucC / \nucC\nucG\/ pairs, 20\% \nucA\nucU / \nucU\nucA\/ pairs, and 10\% Wobble pairs.
This baseline performs surprisingly well and even surpasses both T5 models at moderate sampling budgets. 
Although it 
ultimately is far below the best model, its competitiveness underscores the limitations of uninitialized models in capturing structural constraints.
%Overall, the results show that pretrained decoder-only LMs adapted to RNA tokens provide a much stronger foundation for conditional RNA sequence generation than models trained from scratch. 
%Pretrained adaptation substantially improves sample quality, scaling behavior, and the effectiveness of the RL stage that follows.

To evaluate how different supervised-learning (SL) training corpora affect downstream RNA design, we train the pretrained Qwen2.5-0.5B model on three sources of structure--sequence pairs—Eterna-web, Rfam-Learn-MFE, and Random-MFE, and measure performance on Eterna100 and RNAsolo100, comparing with the full model trained on the %union of all three datasets, corresponding to our 
full supervised training set \YXtrain. 
%As shown in 
Table~\ref{fig:sl_plot_with_table}(b) shows
that
% each dataset yields different performance levels. 
training on Eterna-web works best on Eterna100 ($0.51$) and training on Random MFE works best on RNAsolo100 ($0.71$).
%, and Rfam-Learn-MFE produces intermediate performance on both benchmarks. 
The combined model achieves the best overall results across both datasets ($0.54$ on Eterna100 and $0.72$ on RNAsolo100), indicating that %aggregating 
heterogeneous structural sources provide complementary coverage.
 %and significantly improves generalization.


%Overall, these results show that while individual datasets capture distinct structural biases, combining them produces the most robust SL initialization for subsequent reinforcement learning.


\begin{figure*}[t]
%=======
%\begin{figure}[b]
%>>>>>>> f5dfd48a36ecc8f2def9567d11b632de84917f1f
  \centering
  % Left: figure
  \begin{tabular}{cc}
  \raisebox{3cm}{(a)}
  \begin{minipage}[t]{0.4\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/best_of_N_probability.pdf}
    % \caption{}  % no separate caption here if you want a single joint one below
  \end{minipage}
  &
  % Right: table
  \raisebox{4cm}{
  (b) \hspace{-0.4cm}
  \begin{minipage}[t]{0.55\textwidth}
    \centering
     \begin{tabular}{|l||r|r||c|c|}
      \hline
      {SL training data} & \textbf{$|\{\vecystar\}|$} & \textbf{$|\{\vecystar,\vecx\}|$} & {Eterna100} & {RNAsolo100} \\ \hline
      \Eternaweb       & 9.3K   & 0.9M  & 0.51 & 0.70 \\
      \RfamlearnMFE    & 51.1K  & 1.1M  & 0.46 & 0.67 \\
      \RandomMFE       & 100K   & 1.0M    & 0.47 & 0.71 \\
      \hline
      All (\YXtrain)   & 160.4K & 3.0M    & 0.54 & 0.72 \\
      \hline
    \end{tabular}
    %\end{table}
    \\
    \caption{Supervised learning results. (a) Comparison of different models trained on \YXtrain in terms of best-of-$N$ Boltzmann probability on Eterna100. (b) Comparison of Qwen-0.5B models trained on different datasets, in terms of 
    best-of-$10^4$ Boltzmann probability on two test sets.  \label{fig:sl_plot_with_table}}
  \end{minipage}
  }	
  \end{tabular}
%  \caption{Comparison of RNADesign on Eterna100 and RNAsolo100 across SL models trained on different data sources, alongside the corresponding performance curve.}
\end{figure*}


%Overall, these results show that while individual datasets capture distinct structural biases, combining them produces the most robust SL initialization for subsequent reinforcement learning.



%
%Figure~\ref{fig:sl_plot_with_table}(a) reports the best-of-$N$ Boltzmann probability achieved by each supervised-learning (SL) model as a function of the number of decoded samples $N$ per target structure. Across all sampling budgets, the pretrained Qwen-0.5B-SL model performs the strongest, reaching a best-of-$N$ probability of approximately $0.55$ at $N=10^4$. In contrast, both scratch-trained models, Qwen-0.5B-SL\_Scratch and T5-0.7B-SL\_Scratch, perform substantially worse, with flatter curves and significantly lower probability values across all $N$. The performance degradation is especially pronounced for the T5-scratch model, whose output remains near baseline even under extensive sampling. These results clearly indicate that training transformer LMs for RNA design entirely from scratch is ineffective regardless of architecture. The \texttt{Target\_Initialization} baseline, derived from direct Watson--Crick--Franklin instantiation, performs surprisingly well and even surpasses both T5 models at moderate sampling budgets. Although it 
%ultimately plateaus far below the Qwen models, its competitiveness underscores the limitations of uninitialized models in capturing structural constraints.
%
%Overall, the results show that pretrained decoder-only LMs adapted to RNA tokens provide a much stronger foundation for conditional RNA sequence generation than models trained from scratch. Pretrained adaptation substantially improves sample quality, scaling behavior, and the effectiveness of the RL stage that follows.
%
%To evaluate how different supervised-learning (SL) training corpora affect downstream RNA design, we train the pretrained Qwen2.5-0.5B model on three sources of structure--sequence pairs—Eterna-web, Rfam-Learn-MFE, and Random-MFE, and measure performance on Eterna100 and RNAsolo100. We also train a model on the union of all three datasets, corresponding to our full supervised training set \YXtrain. As shown in Table~\ref{fig:sl_plot_with_table} 3(b), each dataset yields different performance levels. Eterna-web provides the highest score on Eterna100 ($0.51$), Random MFE achieves the highest score on RNAsolo100 ($0.71$), and Rfam-Learn-MFE produces intermediate performance on both benchmarks. The combined model achieves the best overall results across both datasets ($0.54$ on Eterna100 and $0.72$ on RNAsolo100), indicating that aggregating heterogeneous structural sources provides complementary coverage and 
%significantly improves generalization.
%
%Overall, these results show that while individual datasets capture distinct structural biases, combining them produces the most robust SL initialization for subsequent reinforcement learning.




\vspace{-0.4cm}

\subsection{Decoding: Constrained vs.~Unconstrained}
\vspace{-0.2cm}
We empirically compare naive decoding and constrained decoding on the union test set \Ytest using the supervised-only Qwen2.5-0.5B model.  
For each target structure, we draw $10^3$ samples with both methods and, for every decoded sequence, record (i) length mismatch (sequence length $\neq |\vecystar|$), (ii) structural invalidity (any base pair in $\vecystar$ violating Watson--Crick--Franklin or wobble rules), and (iii) wall-clock decoding time.

As shown in Fig.~\ref{fig:combined_metrics_vs_length}, naive decoding leads to growing length mismatch and a sharp increase in invalid sequences for longer targets, wasting a substantial fraction of samples.  
Constrained decoding, by contrast, eliminates both mismatch and invalidity by design, 
while incurring a modest $\sim30\%$ 
overhead. %increase in decoding time.  
This small overhead is outweighed by the gain in effective sample efficiency, so we adopt constrained decoding 
in RL.
%in all subsequent experiments.

\vspace{-15pt}
\begin{figure}[h] 
    \centering
    \includegraphics[width=0.8\textwidth]{figs/combined_metrics_vs_length.pdf}
    \vspace{-8pt}
    \caption{Naive decoding vs.~constrained decoding on the Union Test Set \Ytest, with $10^3$ samples per structure, using the model after supervised learning. Naive decoding produces large amount of invalid designs, especially for longer structures, while constrained decoding guarantees validity, with the cost of being $\sim$30\% slower.}
    \label{fig:combined_metrics_vs_length}
\end{figure}

\vspace{-0.3cm}

\subsection{Reinforcement Learning}

Fig.~\ref{fig:SL+RL} shows that applying reinforcement learning (RL) on top of the 
supervised-learning (SL) model leads to a substantial improvement in best-of-$N$ Boltzmann probability 
across all three benchmarks. The RL-enhanced model consistently outperforms the SL-only model, with 
particularly large gains on Eterna100 and Rfam-Taneda-27, where the performance gap remains pronounced 
for all sampling budgets. 
%On RNAsolo100, RL provides a smaller but still measurable improvement, and the 
%RL curve approaches or matches the SOTA performance even at moderate sample sizes.

Overall, these results demonstrate that RL significantly strengthens the model’s ability to generate 
high-probability designs, especially for benchmarks involving complex or human-designed structures, and 
consistently improves the scaling behavior of the SL baseline. Similarly, from Table~\ref{tab:comparison-eterna100-rnasolo100}, we observe that our reinforcement-fine-tuned model consistently matches or surpasses other methods on ensemble-based metrics. It also achieves the best performance on $p(\vecy | \vecx)$ accross all datasets and attains the best NED—tied only with SAMFEO on RNAsolo100 and Rfam\text{-}Taneda\text{-}27.



\begin{figure*}[h]
  \centering
  \vspace{-0.4cm}
  \hspace{-0.3cm}
  \begin{tabular}{ccc}
    \includegraphics[width=0.33\linewidth]{figs/best_of_N_probability_eterna.pdf}
    &
    \includegraphics[width=0.33\linewidth]{figs/best_of_N_probability_RNAsolo.pdf}
    &
    \includegraphics[width=0.33\linewidth]{figs/best_of_N_probability_rfam.pdf}
    \\[-0.2cm]
    (a) Eterna100 & (b) RNAsolo100 & (c) Rfam-Taneda-27
  \end{tabular}
  \vspace{-0.2cm}
\caption{Best-of-$N$ probability curves for the SL and SL+RL models on three test sets.
In all cases,
RL brought substantial improvements over SL,
surpassing SOTA (SAMFEO).
See Fig.~\ref{fig:SI-SL+RL} in Appendix for other metrics.\label{fig:SL+RL}}
\end{figure*}


\begin{table}[h]
\centering
\resizebox{.49\textwidth}{!}{
\begin{tabular}{l|cccc|cccc}
\hline
\multirow{2}{*}{Method} 
    & \multicolumn{4}{c|}{\textbf{Eterna100}} 
    & \multicolumn{4}{c}{\textbf{RNAsolo100}} \\
\cline{2-9}
    & $p(\vec{y}^\star\mid\vec{x})\!\uparrow$
    & NED$\downarrow$
    & MFE$\uparrow$
    & uMFE$\uparrow$
    & $p(\vec{y}^\star\mid\vec{x})\uparrow$
    & NED$\downarrow$
    & MFE$\uparrow$
    & uMFE$\uparrow$ \\
\hline
RNAinverse-pf 
    & 0.571 & 0.045 & 77 & 72
    & 0.710 & 0.015  & 79 & 79 \\
NEMO 
    & 0.271 & 0.098 & \textbf{79} & \textbf{77}
    & 0.506 & 0.038 & \textbf{81} & \textbf{81} \\
SAMFEO 
    & 0.580 & 0.043 & 77 & 74
    & 0.723 & \textbf{0.013} & 80 & 79 \\
\hline
{Ours: SL+RL} 
    & \textbf{0.588} & \textbf{0.039} & 75 & 73
    & \textbf{0.728} & \textbf{0.013} & \textbf{81} & \textbf{81} \\
\hline
\end{tabular}%\\[0.1cm]
}
\hspace{3pt}
%\caption{Comparison of RNA design methods evaluated on Eterna100 and RNAsolo100.}
%\label{tab:comparison-eterna100-rnasolo100}
%\end{table}
%\begin{table}[h!]
\centering
\resizebox{.49\textwidth}{!}{
\begin{tabular}{l|cccc|cccc}
\hline
\multirow{2}{*}{Method} 
    & \multicolumn{4}{c|}{\textbf{Eterna100-v2}} 
    & \multicolumn{4}{c}{\textbf{Rfam-Taneda-27}} \\
\cline{2-9}
    & $p(\vec{y}^\star\mid\vec{x})\!\uparrow$
    & NED$\downarrow$
    & MFE$\uparrow$
    & uMFE$\uparrow$
    & $p(\vec{y}^\star\mid\vec{x})\!\uparrow$
    & NED$\downarrow$
    & MFE$\uparrow$
    & uMFE$\uparrow$ \\
\hline
RNAinverse-pf 
    & 0.590 & 0.039 & 82 & 77
    & 0.808   & \textbf{0.004}   & 24 & 24 \\
NEMO 
    & 0.270 & 0.098 & \textbf{90} & \textbf{87}
    & 0.411 & 0.025 & \textbf{25} & \textbf{25} \\
SAMFEO 
    & 0.596 & 0.036 & 83 & 79
    & 0.809 & \textbf{0.004} & 24 & 24 \\
\hline
{Ours: SL+RL} 
    & \textbf{0.605} & \textbf{0.033} & 81 & 80
    & \textbf{0.812} & \textbf{0.004} & 24 & 24 \\
\hline
\end{tabular}
}
\vspace{5pt}
\caption{Comparison of our work with state-of-the-art systems on
all four test sets.
% Eterna100-v2  and Rfam-Taneda-27.}
\label{tab:comparison-eterna100-rnasolo100}}
%>>>>>>> 65909b4cee617b69c55fb00f8cab361320a101fa
\end{table}

 % This metric measures the thermodynamic probability of the target structure under the best sample among $N$ candidates and reflects the intrinsic quality of the SL initialization prior to reinforcement learning (RL).


==> framework.tex <==
% !TEX root = main.tex

%Unlike many RNA design methods~\citep{portela:2018unexpectedly,Zadeh+:2010} that focus on either one \MFE criterion or one ensemble property, our goal is to perform RNA design for both ensemble- and \MFE-based criteria jointly. 
Unlike exsiting RNA design methods~\citep{portela:2018unexpectedly,Zadeh+:2010,garcia+:2013rnaifold,runge2018learning} focusing  a single \MFE-based or ensemble metric, our goal is to perform RNA design by jointly optimizing both ensemble- and \MFE-based criteria.
%Following our prior work SAMFEO~\citep{zhou+:2023samfeo}, our algorithm first leverage motif-level divide-conquer-combine strategy to efficiently optimizes equilibrium  probability (Eq.~\ref{eq:prob}) or NED (Eq.~\ref{eq:ned}) for a given target structure $\ystar$ and yields \MFE or \UMFE solutions as byproducts, which will be introduced in Section~\ref{sec:motif-level}.
For a given target structure $\ystar$, we first employs a motif-level divide–conquer–combine strategy to efficiently optimize equilibrium probability $p(\ystar \mid \vecx)$ (Eq.~\ref{eq:prob}). This process simultaneously produces \MFE-based designs and \NED-based designs as byproducts, which will be detailed in Section~\ref{sec:motif-level}.
Then, we introduce a novel rival search algorithm (described in Section~\ref{sec:rival-serach}) to further refine the sequences obtained from ensemble optimization, yielding additional \MFE and \UMFE solutions.
The overall workflow of our approach is depicted in Fig.~\ref{fig:framework}.
\vspace{-0.5cm}
\begin{figure}[h]
\centering
\resizebox{0.8\textwidth}{!}{
	\begin{tikzpicture}[node distance=1.0cm]
	\node (input) [input] {input $\ystar$};
	\node (motif_level) [process, right=of input, xshift=-0.7cm, align=center] {motif-level \\ divide-conquer-combine};
	\node (ensemble) [right=of motif_level, align=center] {$p(\ystar \mid \vecx)$ \\ designs};
	\node (structure_level) [process, right=of ensemble, align=center] {structure-level \\ rival search};
	\node (optional) [output, above=of structure_level, align=center, yshift=-1cm] {(optional)};
	\node (output) [output, below=of motif_level, yshift=-0.2cm] {\MFE \& \UMFE \&  \NED designs};
	\node (fbest)  [output, below=of structure_level, yshift=-0.2cm] {more \MFE \& \UMFE designs};
	
	
	\draw [arrow] (input) -- (motif_level);
	\draw [arrow] (motif_level) -- node[above] {} (ensemble);
	\draw [arrow] (ensemble) -- node[above] {} (structure_level);
	\draw [arrow] (motif_level) -- (output) node[midway,right] {byproduct};
	\draw [arrow] (structure_level) -- (fbest) node[midway,right] {satisfaction};	
	\end{tikzpicture}
}
\caption{Overview of our RNA design framework.}\label{fig:framework}
\end{figure}


==> introduction.tex <==
% !TEX root = main.tex

%\section{Introduction}
Ribonucleic acid (RNA) plays a central role in cellular processes such as transcription, translation, catalysis, and gene regulation~\cite{eddy:2001,doudna+cech:2002,bachellerie+:2002}. 
Its biological and biomedical importance is underscored by RNA viruses like SARS-CoV-2, as well as the Nobel Prizes in Physiology or Medicine awarded in 2023 for mRNA vaccine technologies and in 2024 for the discovery of microRNAs.  
Since structure determines function, designing artificial RNA molecules with specific secondary structures enables a wide range of applications, including artificial ribozymes~\cite{dotu+:2014,yamagami+:2018}, microRNAs~\cite{schwab+:2006}, aptamers~\cite{hamada:2018}, and riboswitches~\cite{bauer+suess:2006,findeiss+:2017}.  

The problem of \emph{RNA design}, also known as RNA inverse  folding, aims to find an RNA sequence that folds into a given target structure~\cite{hofacker+:1994,andronescu+:2004,garcia+:2013rnaifold,zadeh+:2011nupack,zhou+:2023samfeo}. 
Computationally, this is an exceptionally challenging problem due to two levels of combinatorial explosion,
both in the {\em sequence (design) space} and {\em structure (folding) space}.  
For any target structure, there are exponentially many candidate designs,
while for each design, there are also exponentially many alternative structures that compete with the target.  
Indeed, the problem has been proven NP-hard under simplified energy models~\cite{bonnet+:2020}.  

Existing approaches to RNA design 
can be broadly categorized into three camps.
%rely on heuristic or optimization-based search.  
The most common one is heuristic local search that iteratively mutates candidate sequences, such as RNAinverse~\cite{hofacker+:1994}, NEMO~\cite{portela:2018nemo} and SAMFEO~\cite{zhou+:2023samfeo}.
Operating on one or a few sequences at a time,
they cannot keep up with the exponential growth of the design space and struggle at long and hard-to-design structures.
To address this fundamental problem,
the second camp recursively decomposes large structures
into smaller ones,
which includes
RNA-SSD~\cite{andronescu+:2004}, RNAiFold~\cite{garcia+:2013rnaifold},
and NUPACK~\cite{zadeh+:2011nupack}.
Nevertheless, these methods are computationally expensive, 
and generally underperform the first camp.
A third group uses  
reinforcement learning (RL), formulating RNA design as a sequential decision-making problem~\cite{eastman+:2018,runge+:2019,obonyo+:2022}.  
However, the performance of 
 these vanilla RL systems trained from scratch
%led to 
% These methods demonstrated that an agent can learn heuristics for sequence construction, but they suffer from sparse reward signals, unstable optimization, and 
%performance that 
lag behind strong heuristic designers.  

In this work, we propose a fundamentally different perspective: RNA design as \emph{conditional sequence generation}.  
Instead of solving a combinatorial optimization problem from scratch for each structure, we learn a reusable (shared) \emph{neural approximator solver}.  
We make the following contributions:
\begin{enumerate}
\item We formulate RNA design as conditional sequence generation using an autoregressive language model.
%(LM) mapping target structures to candidate sequences.
\item We devise a constrained decoding algorithm to ensure the validity of  designs for the input structure.
\item We develop a unified framework that combines  pretraining, supervised learning (SL) on 
%large amounts of 
structure–sequence pairs,  
and reinforcement learning (RL) 
on selected structures to directly optimize folding success.  
\item We carefully construct the training set for SL to avoid test set contamination and overfitting, 
and develop methods to generate large amounts of high quality structure-sequence pairs. We also develop methods to select a small subset of structures for efficient RL based on the diversity of samples.
\item We utilize
%we amortize the design cost across many tasks, and
 %enabling 
 fast parallel sampling of large amounts of designs on modern GPUs,
 and our best designs outperform (or tie with) the state-of-the-art systems in key ensemble-based metrics on all four test sets.
%\item
%This approach provides an alternative paradigm to traditional RNA design methods, outperforming the state-of-the-art in terms of ensemble-based metrics on all four test sets.
\end{enumerate}
%, matching their performance while offering 
%significant
%orders-of-magnitude 
%efficiency gains.  

==> methods.tex <==
% !TEX root = main.tex

%\section{Methods}

\subsection{RNA Design as Conditional Sequence Generation}

We frame RNA design as a conditional sequence generation task.  
Given a target secondary structure~$\vecystar$, the objective is to generate a nucleotide sequence $\boldsymbol{x}$ that folds into $\vecystar$.  
To this end, we employ an autoregressive language model $\LM{\theta}$ parameterized by $\theta$ that defines the conditional distribution

\vspace{-8pt}
\[
p_\theta(\boldsymbol{x} \mid \vecystar) 
= \prod_{t=1}^{n} p_\theta(x_t \mid \vecx_{<t}, \vecystar),
\]
where $x_t \in \mathcal{N}$ is the nucleotide at position $t$ and $\vecx_{<t}$ is the sequence prefix.  
This autoregressive factorization enables the model to condition each nucleotide decision on both the target structure and the previously generated prefix, capturing local dependencies that influence valid folding.

\paragraph{Vocabulary and input.}
We employ a compact, domain-specific vocabulary designed for structure-conditioned RNA generation.  
It consists of the four nucleotides (\nucA, \nucC, \nucG, \nucU), the three dot–bracket structure symbols (\texttt{(}, \texttt{)}, \texttt{.}), and a small set of control tokens.  
The tokens \texttt{<struct>} and \texttt{</struct>} delimit the target structure, while \texttt{<bos>} and \texttt{<eos>} mark sequence boundaries.  
This minimal vocabulary ensures stable training and allows the model to directly map structural prompts to nucleotide outputs.
During inference, the structure is provided as a prefix prompt:

\vspace{-10pt}
\[
\texttt{<struct> ( . ( . . . ) ) </struct> <bos>}
\]
after which the model autoregressively emits nucleotides until producing an \texttt{<eos>} token:

\vspace{-10pt}
\[
\texttt{G A C U U A G C <eos>}.
\]


\subsection{Constrained Decoding}
\label{sec:decoding}

Autoregressive generation with a language model does not, by default, respect the biochemical pairing rules required for a sequence to be compatible with a given RNA secondary structure.  
When decoding nucleotides token by token, the model may freely emit bases that violate Watson--Crick--Franklin or wobble pairing at positions that correspond to paired sites in $\vecystar$, resulting in invalid sequences outside the valid design space $\mathcal{X}(\vecystar)$. 
To mitigate this mismatch between vanilla language model generation and RNA thermodynamic constraints, we employ a \emph{constrained decoding} mechanism that enforces base-pairing rules during generation.


In the aspect of formal language theory, our valid design space $\mathcal{X}(\vecystar)$ is a {\bf context-free language} (with long-distance dependencies) and needs a runtime stack to ensure valid decoding. However, our method below uses a (stack-based) precomputation to avoid the runtime stack, reducing the overhead.

\paragraph{Constraint rule.}
Let $\vecystar$ denote a dot–bracket structure of length~$n$.  
We precompute a mapping $m(t)$ that associates each closing parenthesis with its corresponding opening partner.  
At decoding step~$t$, the set of admissible nucleotides is defined as:

\vspace{-15pt}
\[
\mathcal{A}_t =
\begin{cases}
\{\nucA, \nucC, \nucG, \nucU\}, & y^\star_t\!\in\!\{\texttt{.},\texttt{(}\},\\
\mathrm{Comp}(x_{m(t)}), & y^\star_t\!=\!\texttt{)},\\
\{\texttt{<eos>}\}, & t>n,
\end{cases}
\]
where $\mathrm{Comp}(\cdot)$ enumerates nucleotides compatible with Watson–Crick–Franklin or wobble pairing:

\vspace{-10pt}
\[
\mathrm{Comp}(\nucA)=\{\nucU\},\;
\mathrm{Comp}(\nucC)=\{\nucG\},\;
\mathrm{Comp}(\nucG)=\{\nucC, \nucU\},\;
\mathrm{Comp}(\nucU)=\{\nucA, \nucG\}.
\]

\vspace{-20pt}
\paragraph{Implementation.}
At each decoding step, we mask the logits of all invalid nucleotides according to $\mathcal{A}_t$ and renormalize:
\(
\tilde{p}_\theta(x_t \mid \vecx_{<t},\vecystar)
\propto 
\mathbf{1}[x_t\!\in\!\mathcal{A}_t]\,
p_\theta(x_t \mid \vecx_{<t},\vecystar).
\)
A lightweight callback computes $\mathcal{A}_t$ on-the-fly from $y^\star_t$ and the nucleotide previously generated at its paired site.  
After position $n$ has been filled, only \texttt{<eos>} remains valid, ensuring that the generated sequence length matches the target structure.

\paragraph{Effect.}
This decoding strategy guarantees structural validity by construction and reduces the effective search space from $4^n$ (regular language $\{\nucA,\nucC,\nucG,\nucU\}^n$) to $6^m 4^u$ (context-free language $\mathcal{X}(\vecystar)$) for $m$ base pairs and $u$ unpaired positions.  
Its computational overhead is about 30\% (see Fig.~\ref{fig:combined_metrics_vs_length}), yet it substantially improves sample efficiency and training stability in both supervised and reinforcement learning settings.


==> prelim.tex <==
% !TEX root = main.tex

%\section{Preliminaries}
\vspace{-0.2cm}
\subsection{RNA Sequences and Structures}

An RNA sequence $\vecx$ of length $n$ is a string of nucleotides 
$x_1 x_2 \dots x_n$, where $x_i \in \mathcal{N}$ and 
$\mathcal{N} \stackrel{\Delta}{=} \{\texttt{A}, \texttt{C}, \texttt{G}, \texttt{U}\}$.  
A pseudoknot-free secondary structure $\vecy$ is represented as a dot-bracket string of the same length.  
Each character $y_i \in \{ \texttt{.}, \texttt{(}, \texttt{)}\}$ indicates whether nucleotide $x_i$ is unpaired, paired downstream, or paired upstream, respectively.  
Base pairs are restricted to Watson–Crick–Franklin or wobble pairs:  
$\mathcal{P} = \{ \texttt{CG}, \texttt{GC}, \texttt{AU}, \texttt{UA}, \texttt{GU}, \texttt{UG}\}$.  
For a given sequence $\vecx$, its \emph{ensemble} $\mathcal{Y}(\vecx)$ consists of all possible secondary structures.  
In thermodynamic RNA folding models, \emph{Gibbs free energy change} $\Delta\:\!\! G^{\scriptsize\circ\!}(\vecx, \vecy)$ is used to characterize the stability of secondary structure $\vecy \in \mathcal{Y}(\vecx)$. The lower the free energy~$\Delta\:\!\! G^{\scriptsize\circ\!}(\vecx, \vecy)$, the more stable the structure $\vecy$ for $\vecx$. The structure with the \emph{minimum free energy} is the most stable structure in the ensemble, i.e., 
the {\em \text{MFE} structure},
%
\vspace{-5pt}
\begin{equation}
\text{MFE}(\vecx) \stackrel{\Delta}{=} \argmin_{\vecy \in \mathcal{Y} (\vecx)} \Delta\:\!\! G^{\scriptsize\circ\!}(\vecx, \vecy).
\vspace{-5pt}
\end{equation}

Note that for most methods for secondary structure prediction, ties for $\argmin$ are broken arbitrarily when there are multiple lowest free energy structures.
This issue was often neglected in the literature, but it deserves clarification here. To be precise, we define 
%\begin{equation}
\(\MFEs(\vecx) \stackrel{\Delta}{=} \{\vecy \mid 
\Delta\:\!\! G^{\scriptsize\circ\!}(\vecx, \vecy) = \min_{\vecy' \in \mathcal{Y}(\vecx)} \Delta\:\!\! G^{\scriptsize\circ\!}(\vecx, \vecy')\}\)
%\end{equation}
to be the {\em set of MFE structures} for $\vecx$. When 
$|\MFEs(\vecx)|=1$,
we say $\vecx$ has a {\em unique MFE} (uMFE) structure. 

The \emph{partition function} 
%\begin{equation}
\(
Q(\vecx) \stackrel{\Delta}{=}  \sum_{\vecy \in \mathcal{Y}(\vecx)} e^{-\Delta\:\!\! G^{\scriptsize\circ\!}(\vecx, \vecy)/RT}
\)
sums the contribution of all structures in the ensemble,
%\end{equation}
where $R$ is the molar gas constant and $T$ is the absolute temperature. Accordingly, the Boltzmann 
%equilibrium 
probability of a sequence $\vecx$ folding into a structure $\vecy$ is defined as
\(%begin{equation}
p(\vecy \mid \vecx) = \frac{e^{-\Delta\:\!\! G^{\scriptsize\circ\!}(\vecx, \vecy)/RT}}{Q(\vecx)}.
\)%end{equation}

\vspace{-0.2cm}
\subsection{RNA Design Problem}

Given a target structure~$\vecystar$, RNA design aims to find a suitable RNA sequence~$\vecx$ 
that can naturally and easily fold into $\vecystar$,
within the design space $\mathcal{X}(\vecystar)$ 
%the set 
of all valid sequences for $\vecystar$:


\vspace{-8pt}
\begin{equation}
\mathcal{X}(\vecystar) \stackrel{\Delta}{=} \{ \vecx \in \mathcal{N}^{|\vecystar|} \mid \forall (i,j)\in \mathit{pairs}(\vecystar), x_i x_j \in \mathcal{P}\}
\end{equation}
We formulate the RNA design problem as optimizing  
a scoring function
$f(\vecx, \vecystar)$ 
over the design space $\mathcal{X}(\vecystar)$:

\vspace{-10pt}
\begin{equation}
\vecxstar = \argmax_{\vecx \in \mathcal{X}(\vecystar)} f(\vecx, \vecystar)
\end{equation}
where
the scoring function quantifies how ``easily'' 
$\vecx$ folds into $\vecystar$. In practice, the literature
\cite{anderson+:2016,zhou+:2023samfeo,tang+:2024} evaluates RNA design 
using several standard metrics which we adopt below.
%thermodynamics-based and structure-based 
%criteria that measure how 
%well a candidate sequence folds into the target structure. We adopt the same 
%standard metrics below. 
The first two (ensemble-based)
are considered more important than the last two (MFE-based),
because even if \vecx is an MFE solution there can still be many  structures with similar energies,
resulting in arbitrarily low probability of \vecystar in ensemble.

\vspace{-5pt}
\begin{itemize}
    \item \textbf{Boltzmann probability} \( p({\vecystar} \mid \vecx) \) meansures
 how likely \( \vecx \) folds into 
    \( {\vecystar} \) among all possible structures.

    \item \textbf{Normalized Ensemble Defect} \( \text{NED}(\vecx, {\vecystar}) \)
     quantifies how well the ensemble of structures formed by \( \vecx \) 
    aligns with the target, penalizing competing folds~\cite{zadeh+:2011}:
%    \begin{equation}
 \(       \text{NED}(\vecx, {\vecystar}) 
        = \frac{1}{|\vecx|} \sum_{\vecy \in \mathcal{Y}(\vecx)} 
        p(\vecy \mid \vecx)\, \dstruct({\vecystar}, \vecy),
  \) %  \end{equation}
    where 
    $\dstruct(\vecy, \vecy') \stackrel{\Delta}{=} 
        |\vecy| 
        - 2 \cdot |\mathit{pairs}(\vecy) \cap \mathit{pairs}(\vecy')|
        - |\mathit{unpaired}(\vecy) \cap \mathit{unpaired}(\vecy')|$ is the structural distance.
   \item {\bf MFE solution}: $f(\vecx,\vecystar)=1$ if $\vecystar\in \MFEs(\vecx)$ else $0$.
   \item {\bf \UMFE solution}: $f(\vecx,\vecystar)=1$ if $\vecystar\in \MFEs(\vecx)$ and $|\MFEs(\vecx)|=1$ else $0$.
   
        %between two structures .
%    and equivalently in base-pairing probability form:
%    \begin{equation}
%        \text{NED}(\vecx, {\vecystar}) 
%        = 1 - \frac{2}{|\vecx|} 
%        \sum_{(i, j) \in \mathit{pairs}({\vecystar})} p_{ij} 
%        - \frac{1}{|\vecx|} 
%        \sum_{j \in \mathit{unpaired}({\vecystar})} q_j,
%    \end{equation}
%    where \( p_{ij} \) is the base-pairing probability, and 
%    \( q_j = 1 - \sum_i p_{ij} \) is the probability that \( j \) is unpaired.

%    \item \textbf{Structural Distance} \( d({\vecystar}, \text{MFE}(\vecx)) \): 
%    This measures the difference between the target structure and the MFE structure of 
%    the designed sequence:
%    \begin{equation}
%        d(\vecy, \vecy') \stackrel{\Delta}{=} 
%        |\vecy| 
%        - 2 \cdot |\mathit{pairs}(\vecy) \cap \mathit{pairs}(\vecy')|
%        - |\mathit{unpaired}(\vecy) \cap \mathit{unpaired}(\vecy')|.
%    \end{equation}

\end{itemize}

==> related.tex <==
% !TEX root = main.tex
\vspace{-0.2cm}
\paragraph{Language Models for RNA Analysis}
Several recent studies %treat RNA as a ``language’’ and
train BERT-style encoders on large RNA corpora for downstream 
structure-prediction and analysis,
including RNABERT, RNA-FM, RNA-MSM,and RiNALMo
% are pretrained %with masked-token objectives
% on millions of RNA sequences and then fine-tuned for downstream tasks~
% 
\cite{RNABERT,RNA-FM,RNA-MSM,RiNALMo}.  
Other encoder-based LMs specialize in particular modalities, such as  BERT-RBP for RNA–protein interaction prediction~\cite{BERT-RBP} and StructmRNA for joint mRNA sequence–structure representation~\cite{StructmRNA}.
%, and lncRNA-specific models for functional classification.  
Benchmarks~\cite{zablocki+:2025} show that such RNA LMs improve analysis, but they (a) operate on RNA sequences without structure tokens, and (b) are encoder-only architectures  and thus incapable of {\em de novo} design.
By contrast, we use a decoder-only LM that conditions on dot–bracket structures and is trained end-to-end to \emph{generate} RNA sequences, with constrained decoding and RL explicitly targeting folding success.

\vspace{-0.1cm}
\paragraph{Generative Models for RNA Generation}
Deep generative models have recently been explored for RNA sequence design.  
GAN- and VAE-style approaches such as RNAGEN and RfamGen generate family- or target-specific RNAs by learning over aligned sequence ensembles, often guided by external predictors or consensus structures~\cite{RNAGEN,RfamGen}.  
Closer to our setting, GenerRNA is an autoregressive LM pretrained on large-scale RNA data and fine-tuned to generate functional (e.g., protein-binding) RNAs
%, for example protein-binding aptamers, 
but without conditioning on an explicit input~\cite{GenerRNA}.
RNAtranslator models protein-conditional RNA design as a sequence-to-sequence problem, where an encoder processes a protein sequence and a decoder generates RNA binders 
%validated by docking and molecular simulations
~\cite{RNAtranslator}.  
%<<<<<<< HEAD
%=======
%
%\begin{comment}
%>>>>>>> 07b02b4146e311a8e72e21892935e72e6e6c3b29
Our LM differs from these generative approaches in three ways.  
First, we condition directly on %dot–bracket 
secondary structures.
%, enabling flexible inverse folding for arbitrary targets.
% without requiring protein partners or tertiary contact maps.  
Second, we enforce base-pairing constraints %\emph{during} generation 
via constrained decoding %to ensure validity 
rather than filtering post hoc.
%, so the output designs are structurally valid by construction rather than filtered post hoc.  
Third, we fine-tune the LM with RL on 
%thermodynamic 
rewards %that combine Boltzmann probability and MFE uniqueness, 
that align with  
%the generator with the 
standard RNA design objectives. 
% rather than only proxy scores such as binding affinity or expression.
%\end{comment}

\vspace{-.1cm}
\paragraph{Reinforcement Learning for RNA Design}
%RL has been extensively explored for RNA design by casting inverse folding as a sequential decision process.  
%Eastman et al.~\cite{eastman+:2018} first showed that a graph-convolutional RL agent can design sequences that fold to a target secondary structure, achieving strong performance on benchmarks such as Eterna100.  
%Runge et al.\ proposed LEARNA and Meta-LEARNA, which use deep RL and meta-learning to train policies across thousands of design tasks so that a single policy can generalize to new targets~\cite{runge+:2019}.  
%Subsequent work introduced self-play RL (RNASP)~\cite{obonyo+:2022}.

Reinforcement learning provides an appealing framework for RNA design by framing it as a sequential decision process: at each step, an agent chooses an action (an edit on the sequence) and receives a reward based on how well the new sequence folds to the target structure.  
Eastman et al.~\cite{eastman+:2018} pioneered this idea,
with each state being a full sequence and each action being an edit on one or two nucleotides.
%using a graph convolutional network policy that sequentially constructs sequences and is rewarded according to the distance between the predicted MFE structure and the target.  
%Their method demonstrated that RL can discover effective, human-competitive heuristics for RNA design.
Runge et al.\ introduced LEARNA and Meta-LEARNA~\cite{runge+:2019}, 
where each state is a partial sequence 
and each action is to add one or two nucleotides. 
%which use deep RL to design full sequences from scratch and leverage meta-learning across tens of thousands of design tasks to obtain policies that generalize to unseen targets~\cite{runge+:2019}.  
Obonyo et al.\ proposed RNASP, a self-play RL framework inspired by AlphaZero 
%that iteratively improves its policy by generating and evaluating sequences against a folding oracle, showing gains on some benchmarks relative to earlier RL baselines
~\cite{obonyo+:2022}.  
Partial RNA design~\cite{runge+:2024} extends LEARNA to 
handle wildcards.
%generalizes the classical inverse folding formulation by defining design tasks over RNA motifs with wildcards in sequence and structure, and separates the design space from the objectives.  
%Based on this formulation, libLEARNA extends LEARNA with masked training and automated RL to efficiently explore large, partially constrained design spaces.  
%These methods demonstrate that RL can handle rich constraint sets and multi-objective formulations, but they still require substantial environment interaction per task and often rely on a folding engine inside the RL loop to evaluate each candidate sequence.

%\begin{comment}
Our use of RL is complementary and operates in a different regime.  
Rather than training a task-specific RL agent from scratch, we fine-tune a \emph{single} structure-conditioned LM that has already been trained by supervised learning on solver-generated examples.  
%Constrained decoding collapses the search space to valid sequences, which alleviates reward sparsity, and GRPO-based policy gradients provide a lightweight mechanism to align the LM with thermodynamic design objectives.  
As a result, our model acts as an amortized neural solver: once trained, it can rapidly generate high-quality designs for new targets without per-instance RL optimization, while still benefiting from RL’s ability to directly optimize folding-based rewards (see also Tab.~\ref{tab:SI-RL}).
%\end{comment}







==> training.tex <==
% !TEX root = main.tex
\subsection{Pretrained Model}


Large language models trained on massive, diverse text corpora have been shown to acquire broad inductive biases that transfer surprisingly well beyond natural language~\cite{touvron+:2023,yang+:2024}.  
Even relatively small decoder-only LMs develop stable attention patterns, long-range dependency modeling, and useful parameter initializations that make fine-tuning in downstream tasks significantly more data-efficient than training a transformer from scratch.  
Motivated by these observations, we begin with the Qwen2.5--0.5B~\cite{yang+:2024} pretrained model as the backbone for our RNA design system.  
Although the original training domain is textual, our experiments show that the pretrained backbone provides substantially better optimization stability and sample efficiency than a randomly initialized transformer of identical architecture.  
In ablations, the scratch-trained model converges more slowly and yields lower folding performance, confirming that the pretrained initialization is a critical component of our approach.

\paragraph{Surgery for RNA adaptation.}
To turn the general-domain LLM into an RNA-capable generator, we perform a minimal architectural modification. As illustrated in Fig.~\ref{fig:RNA_LM_surgery}, we keep all transformer backbone layers intact and modify only the input and output layers. The original embedding matrix and LM head are removed, and we introduce downsized, RNA-specific replacements built around the vocabulary defined above. This preserves the pretrained backbone while enabling the model to process RNA tokens and structural prompts.

\vspace{-15pt}
\begin{figure}[h] 
    \centering
    \includegraphics[width=0.75\textwidth]{figs/RNA_LM_surgery.pdf}
	\vspace{-8pt}
    \caption{We convert a general-domain LLM into an RNA-focused generator by keeping the pretrained transformer backbone intact and replacing only the input and output layers. The original embedding and LM head are downsized and reinitialized to support RNA tokens.}
    \label{fig:RNA_LM_surgery}
\end{figure}


\paragraph{Why not use existing RNA LMs?}
Several RNA-focused language models have been proposed, but they are not well suited to our setting (see also Sec.~\ref{sec:related}):


\begin{enumerate}
    \item \textbf{Lack of structural input.}  
    Existing RNA LMs typically operate only on nucleotide sequences and do not accept dot--bracket structures as input, preventing direct structure-conditioned generation for design.

    \item \textbf{Architectural mismatch.}  
     Most publicly available RNA LMs are BERT-style encoders trained with masked-token objectives rather than autoregressive decoders.  
    A GPT-style RNA LM has been reported, but no usable checkpoint has been released \cite{RNA-GPT}.
	
	\item \textbf{Tokenization mismatch.}  
    Existing RNA LMs adopt subword or BPE-style tokenization (e.g., merging adjacent nucleotides into one token, as in some recent generative RNA LMs~\cite{GenerRNA}).  
    This breaks the one-nucleotide-per-token alignment that our constrained decoding rely on, making it much harder to control the validity of the decoded sequence: base-pairing constraints can no longer be enforced cleanly.


    \item \textbf{Software compatibility.}  
    Many RNA LMs are implemented in standalone codebases or lack HuggingFace compatibility, making integration with our constrained decoding and RL training pipeline difficult.
\end{enumerate}



\subsection{Supervised Learning}

To initialize the model, we construct a training corpus of structure–sequence pairs.  
Following the knowledge distillation paradigm, we employ a strong optimization-based solver (SAMFEO~\cite{zhou+:2023samfeo}) to generate sequences for diverse target structures, including benchmark sets such as Eterna100 and randomly sampled structures (see Sec.~\ref{sec:SLdata}).  
The resulting dataset
\(\YXtrain\) 
made of $\{(\vecystar, \vecx)\}$ pairs
serves as supervised training data, where each $\vecx$ is a valid sequence for  $\vecystar$.  
The model is trained by maximum likelihood estimation (MLE):

\vspace{-8pt}
\[
\LSL(\theta) 
= - \sum_{(\vecystar, \vecx) \in \YXtrain} \log p_\theta(\vecx \mid \vecystar).
\]
This stage teaches the model to map structures to sequences, enabling it to rapidly generate plausible designs.  

\vspace{-0.2cm}
\subsection{Reinforcement Learning}

%\subsubsection{Algorithm}

Supervised learning aligns the model with solver-generated sequences but does not directly optimize our thermodynamic objective (e.g., Boltzmann probability $p(\vecystar \mid \vecx)$ and ensemble defect $\ED(\vecx, \vecystar)$).
We therefore fine-tune $\LM{\theta}$ with a simple group-based REINFORCE-style objective~\cite{williams:1992}, often referred to as \emph{Group Relative Policy Optimization} (GRPO)~\cite{shao+2024}.

Given a target structure $\vecystar$, we sample a group of $K$ sequences
\(
\{\vecx_k\}_{k=1}^K \sim p_\theta(\cdot \mid \vecystar)
\)
(using constrained decoding) and compute rewards $R_k = R(\vecx_k, \vecystar)$.
We form a group baseline and standard deviation
\(
b = \tfrac{1}{K} \sum_{k=1}^K R_k, \
\sigma = \mathrm{Std}_k(R_k),
\)
and define a normalized advantage
\(
\hat{A}_k = \frac{R_k - b}{\sigma + \varepsilon}.
\)
The GRPO loss is
\begin{equation}
\mathcal{L}_{\text{GRPO}}(\theta)
= - \mathbb{E}_k \big[ \hat{A}_k \log p_\theta(\vecx_k \mid \vecystar) \big],
\end{equation}
which increases the probability of better-than-average samples within each group and decreases that of worse-than-average ones, on top of the supervised initialization.










\subsubsection{Reward Design}

For reinforcement learning, we map the thermodynamic quantities in Section~\ref{sec:prelim} to a single scalar reward that reflects how well a candidate sequence $\vecx$ folds into the target structure $\vecystar$.
During RL, we always use constrained decoding (Section~\ref{sec:decoding}) so that sampled sequences satisfy the length and base-pairing constraints of $\mathcal{X}(\vecystar)$; the reward is therefore defined over $\vecx \in \mathcal{X}(\vecystar)$.

\paragraph{Reward components.}
For each sampled pair $(\vecx, \vecystar)$, we call an RNA folding engine to obtain the Boltzmann probability $p(\vecystar \mid \vecx)$, the set of MFE structures $\MFEs(\vecx)$, and whether the MFE is unique.
Let $\mathbb{I}[\cdot]$ denote the indicator function.
We define three reward components:
\begin{align}
r_{\text{prob}}(\vecx, \vecystar)
= p(\vecystar \mid \vecx), \quad
r_{\text{mfe}}(\vecx, \vecystar)
=\mathbb{I}\big[\vecystar \in \MFEs(\vecx)\big], \quad
r_{\text{umfe}}(\vecx, \vecystar)
= \mathbb{I}\big[\vecystar \in \text{uMFE}(\vecx)\big].
%&= \mathbb{I}\big[\vecystar \in \uMFEs(\vecx) \; \& \;  |\MFEs(\vecx)| = 1\big].
\end{align}
The first term rewards sequences whose Boltzmann ensemble is concentrated on the target structure.
The second term adds a bonus whenever the target structure appears among the MFE structures of $\vecx$. %, indicating that $\vecystar$ is thermodynamically optimal.
The third term further rewards sequences whose MFE structure is unique, discouraging strong competing alternative folds. Here $\text{uMFE}(\vecx)$ denotes the unique MFE structure if it exists and the empty set otherwise.

\paragraph{Combined reward.}
We combine the three components with simple linear shaping:
\begin{equation}
R(\vecx, \vecystar)
=  0.5*r_{\text{prob}}(\vecx, \vecystar)
+ 0.25*r_{\text{mfe}}(\vecx, \vecystar)
+ 0.25*r_{\text{umfe}}(\vecx, \vecystar),
\quad
\vecx \in \mathcal{X}(\vecystar).
\end{equation}

By construction, $r_{\text{prob}} \in [0,1]$ and $r_{\text{mfe}}, r_{\text{umfe}} \in [0, 0.5]$, so $R(\vecx, \vecystar) \in [0,1]$ and $R(\vecx, \vecystar) = 1$ exactly when the target structure has probability $1$ and is the unique MFE structure.
If the thermodynamic evaluation fails for numerical or library-related reasons, we fall back to a neutral reward $R(\vecx, \vecystar) = 0$, so such rare cases neither strongly encourage nor discourage the policy.



